Response of the CALICE Si-W Electromagnetic Calorimeter Physics Prototype to Electrons

A prototype Silicon-Tungsten electromagnetic calorimeter (ECAL) for an International Linear Collider (ILC) detector was installed and tested during summer and autumn 2006 at CERN. The detector had 6480 silicon pads of dimension 1x1 cm^2. Data were collected with electron beams in the energy range 6 to 45 GeV. The analysis described in this paper focuses on electromagnetic shower reconstruction and characterises the ECAL response to electrons in terms of energy resolution and linearity. The detector is linear to within approximately the 1% level and has a relative energy resolution of (16.6 +- 0.1)/ \sqrt{E(GeV}) + 1.1 +- 0.1 (%). The spatial uniformity and the time stability of the ECAL are also addressed.

==> Alignment.tex <==
\section{Alignment}
\label{sec:align}


==> Calibration.tex <==
\section{ECAL Hardware Performance}
\label{HardPerf}

Summary of the hardware paper - hints on systematics

pads response stability, no of dead cells

Data quality selection



==> Uniformity.tex <==
\section{Correction of gaps}
\label{sec:Uniformity} 
As discussed in the previous section, the energy loss for events within the inter-wafer gaps is 
important: about 15.3~\% in $x$ and 19.4~\% in $y$ for particles impacting  in the centre of the 
gaps. 
In order to recover this loss and to have a more uniform response
of the calorimeter response, a  simple 
method correcting the shower energy as function 
of the position of the shower barycentre,
($\bar{x}$, $\bar{y}$), was investigated.

The fraction of energy lost in the interwafer gaps increases with the shower energy: it varies from
14.8~\%(19~\%) in $x$($y$) at 10~GeV to 16.1~\%(20~\%)   at 30 GeV. The present approach did not 
include however 
this 
energy effect and used  a combined sample of 10, 15 and 20~GeV electrons, equally populated in order to estimate the ECAL response (normalised to the beam energy) as function of $(\bar{x},\bar{y})$. The response is displayed on Figure~\ref{fig:global_gaps_correction_pardef}.  

\begin{figure}[htbp]
  \centering
  \mbox{
    \epsfig{file=eps/Uniformity/cracs.eps,width=0.98\linewidth}
  }
  \caption{\sl Normalised calorimeter response  as function of the shower barycentre coordinates $\bar{x}$ and $\bar{y}$ (in mm), for a combined sample of 10, 15 and 20~GeV electrons. To characterise the $x$ ($y$) response, the events were requested to be outside the inter-wafer gap in $y$ ($x$), leading to an important difference in the number of events for the two distributions, since the $y$ gap is approximately centred on the beam.}
 \label{fig:global_gaps_correction_pardef} 
\end{figure}

The distributions around the inter-wafer gap positions were fitted with Gaussian functions, independently in $\bar{x}$ and $\bar{y}$: 
\begin{displaymath}
\left(1-a_{x} e^{-\frac{(x_{b}-x_{gap})^2}{2{\sigma}_{x}^2}}\right) \cdot
\left(1-a_{y} e^{-\frac{(y_{b}-y_{gap})^2}{2{\sigma}_{y}^2}}\right)
\end{displaymath}
The results of the Gaussian parametrisations  are given in Table~\ref{tab:global_gaps_correction_fits}.  The gap in $x$ is shallower and wider than that in $y$, owing to the staggering of the gaps in $x$.

\begin{table}[htbp]
  \centering
  \begin{tabular}{|c|c|c|c|}
  \hline
         & $x_{gap}$, $y_{gap}$  & $\sigma_x$, $\sigma_y$ & $a_x$, $a_y$\\
  \hline
  $x$ direction  & -30.01  &      4.3       & 0.143      \\
  \hline
  $y$ direction &   -8.4     &    3.19          & 0.198      \\
  \hline
  \end{tabular}
  \caption{Gaussian parametrisation of the inter-wafer gaps.}
  \label{tab:global_gaps_correction_fits}
\end{table}

The corrections are not applied if the barycentre coordinates of the shower are more than $4\sigma$ away from the fitted gap positions. As illustrated in Figure~\ref{fig:global_gaps_scan}, when the gap corrections are applied, the energy loss over the gaps is reduced to a few percent level. 
\begin{figure}[htbp]
  \centering
  \mbox{
    \epsfig{file=eps/Uniformity/Scan-20GeV.eps,width=0.95\linewidth}
  } 
  \caption{Calorimeter response as function of the shower barycentre coordinates ($\bar{x}$, $\bar{y}$),
  for 20~GeV electrons, before  (black triangles) and after the corrections (blue circles) were applied on  the measured energy. }
 \label{fig:global_gaps_scan}
\end{figure}

Figure~\ref{fig:global_gaps_energy} shows the important reduction in the low energy tail  of the energy distribution for 15~GeV electrons. On the same figure, the red histogram represents the energy distribution for the events outside the gaps.  The resolution loss when going from the clean events to all the events, with corrections applied on the energy, is of the order of 10\%.  They apply successfully to all the energies considered.

\begin{figure}[htbp]
  \centering
  \mbox{
    \epsfig{file=eps/Uniformity/energy-20GeV.eps,width=0.7\linewidth}
  } 
  \caption{Energy distribution for 20~GeV electrons in case of : events outside the inter-wafer gaps (red histogram), all events without corrections (black histogram) and all events with corrections (blue circles). The histograms are normalised to the same number of entries, for an easier comparison. }
 \label{fig:global_gaps_energy}
\end{figure}

